An Implantable Piezofilm Middle Ear Microphone: Performance in Human Cadaveric Temporal Bones

Purpose: One of the major reasons that totally implantable cochlear microphones are not readily available is the lack of good implantable microphones. An implantable microphone has the potential to provide a range of benefits over external microphones for cochlear implant users including the filtering ability of the outer ear, cosmetics, and usability in all situations. This paper presents results from experiments in human cadaveric ears of a piezofilm microphone concept under development as a possible component of a future implantable microphone system for use with cochlear implants. This microphone is referred to here as a drum microphone (DrumMic) that senses the robust and predictable motion of the umbo, the tip of the malleus. Methods: The performance was measured of five DrumMics inserted in four different human cadaveric temporal bones. Sensitivity, linearity, bandwidth, and equivalent input noise were measured during these experiments using a sound stimulus and measurement setup. Results: The sensitivity of the DrumMics was found to be tightly clustered across different microphones and ears despite differences in umbo and middle ear anatomy. The DrumMics were shown to behave linearly across a large dynamic range (46 dB SPL to 100 dB SPL) across a wide bandwidth (100 Hz to 8 kHz). The equivalent input noise (0.1-10 kHz) of the DrumMic and amplifier referenced to the ear canal was measured to be 54 dB SPL and estimated to be 46 dB SPL after accounting for the pressure gain of the outer ear. Conclusion: The results demonstrate that the DrumMic behaves robustly across ears and fabrication. The equivalent input noise performance was shown to approach that of commercial hearing aid microphones. To advance this demonstration of the DrumMic concept to a future prototype implantable in humans, work on encapsulation, biocompatibility, connectorization will be required.

==> main/figures.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/sensor.png}
    \caption{\textit{Drum Mic}: Microscopic view of the sensitive part (left) and of all sides of the whole sensor (right).}
    \label{fig:sensor}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/setup.png}
    \caption{Experimental setup.}
    \label{fig:measurement_setup}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/histology.png}
    \caption{Position of the DrumMic in the middle ear. \textit{Left}: Microscopic view of the DrumMic experimentally implanted in a cadaveric middle ear cavity (left ear) through an extended facial recess approach. Due to the individual distance between umbo and promontory and shape of the promontory, the sensor was underlaid and stabilized in this case with additional platforms
    \textit{Right}: Horizontal histology section through a healthy middle ear (H\&E stain) showing a schematic drawing of the DrumMic (black) on the promontory, the Jacobson's nerve on the promontory surface and its relation to the umbo (white arrow)}
    \label{fig:histology}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/fig1.png}
    \caption{\textit{Left:} Umbo displacement normalized to ear canal pressure shown in color for four different bones labeled (A,B,C,D) and five different drum microphones labeled (1,2,3,4,5). The umbo displacements prior to insertion of the drum microphone are plotted with dashed lines, while umbo displacements after drum microphone placement are plotted with solid lines. \textit{Right:} Microphone output normalized to ear canal pressure. The charge output due to noise and electrical pickup are shown in light gray and are in units of output charge only since no acoustic stimulus was administered during these measurements. It is evident from the low frequency umbo magnitude decrease that the insertion of the microphone stiffens the umbo. The sensitivity of the microphone is seen to be agnostic to considerable variation in the umbo displacement and is thus a good proxy for the ear canal pressure.}
    \label{fig:1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/fig2.png}
    \caption{Comparing the sensitivity relative to ear canal pressure and sensitivity to umbo displacement of the same drum microphone, it is evident that good contact is needed for a robust response and change in offset with platform(s) has a large effect on sensitivity re umbo displacement, but results in small changes to sensitivity re ear canal pressure.}
    \label{fig:2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/fig3.png}
    \caption{\textit{Left:} Frequency response of a two microphones in the same ear. \textit{Right:} Response from the same microphone implanted in two different ears. The microphones have similar performance demonstrating consistency in fabrication. The responses of one microphone in different ears are also similar. All microphone responses due to variations in microphones and ears are plotted in \Cref{fig:1}.}
    \label{fig:3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/fig4.png}
    \caption{\textit{Left:} Microphone input-output curves. \textit{Right:} Microphone frequency response. The microphones exhibit good linearity across a large dynamic range (20 dB SPL to 90 db SPL) and wide bandwidth (\SI{0.1}{kHz} to \SI{10}{kHz}). The frequency response of the gain is stable (showing linearity) for large variations of input to the speaker. If the voltage reaches \SI{500}{mV}, some nonlinearity is seen near \SI{1}{kHz} and \SI{3}{kHz}. For our setup, \SI{500}{mV} input to the speaker results in 109 dB SPL at \SI{2}{kHz}.}
    \label{fig:4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/fig5.png}
    \caption{\textit{(Top)} 1/3-Octave normalized A-weighted equivalent input noise (EIN) for two drum microphones as compared to the hearing-aid Knowles microphone. The best and worst noise performance of the drum microphone is shown in pink and blue respectively. The Knowles microphone has a significantly lower noise floor. \textit{Bottom:} EIN bandwidth integrated over 100 Hz to 8 kHz.}
    \label{fig:5}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/fig6.png}
    \caption{\textit{Top:} Noise performance of an ideal drum microphone competitive with current commercial external microphones used in cochlear implants. By making the microphone differential and shielded we can increase sensitivity and reduce noise. If we consider the increase in microphone sensitivity due to the pinna gain the equivalent input noise is further reduced. The shielded EIN is computed using noise measured for a drum microphone on the bench with the line harmonics removed. \textit{Bottom:} The noise bandwidth is integrated over \SI{100}{Hz} to \SI{8}{kHz}.}
    \label{fig:6}
\end{figure}
